Learning Causal Effects on Hypergraphs

Hypergraphs provide an effective abstraction for modeling multi-way group interactions among nodes, where each hyperedge can connect any number of nodes. Different from most existing studies which leverage statistical dependencies, we study hypergraphs from the perspective of causality. Specifically, in this paper, we focus on the problem of individual treatment effect (ITE) estimation on hypergraphs, aiming to estimate how much an intervention (e.g., wearing face covering) would causally affect an outcome (e.g., COVID-19 infection) of each individual node. Existing works on ITE estimation either assume that the outcome on one individual should not be influenced by the treatment assignments on other individuals (i.e., no interference), or assume the interference only exists between pairs of connected individuals in an ordinary graph. We argue that these assumptions can be unrealistic on real-world hypergraphs, where higher-order interference can affect the ultimate ITE estimations due to the presence of group interactions. In this work, we investigate high-order interference modeling, and propose a new causality learning framework powered by hypergraph neural networks. Extensive experiments on real-world hypergraphs verify the superiority of our framework over existing baselines.

==> ref_old.tex <==
%%% ====================================================================
%%%  BibTeX-file{
%%%     author          = "Gerry Murray",
%%%     version         = "1.2",
%%%     date            = "2 April 2012",
%%%     filename        = "acmsmall-sample-bibfile.bib",
%%%     address         = "ACM, NY",
%%%     email           = "murray at hq.acm.org",
%%%     codetable       = "ISO/ASCII",
%%%     keywords        = "ACM Reference Format, bibliography, citation, references",
%%%     supported       = "yes",
%%%     docstring       = "This BibTeX database file contains 'bibdata' entries
%%%                        that 'match' the examples provided in the Specifications Document
%%%                        AND, also, 'legacy'-type bibs. It should assist authors in
%%%                        choosing the 'correct' at-bibtype and necessary bib-fields
%%%                        so as to obtain the appropriate ACM Reference Format output.
%%%                        It also contains many 'Standard Abbreviations'. "
%%%  }
%%% ====================================================================

% Journals

% First the Full Name is given, then the abbreviation used in the AMS Math
% Reviews, with an indication if it could not be found there.
% Note the 2nd overwrites the 1st, so swap them if you want the full name.

 %{AMS}
 @String{AMSTrans = "American Mathematical Society Translations" }
 @String{AMSTrans = "Amer. Math. Soc. Transl." }
 @String{BullAMS = "Bulletin of the American Mathematical Society" }
 @String{BullAMS = "Bull. Amer. Math. Soc." }
 @String{ProcAMS = "Proceedings of the American Mathematical Society" }
 @String{ProcAMS = "Proc. Amer. Math. Soc." }
 @String{TransAMS = "Transactions of the American Mathematical Society" }
 @String{TransAMS = "Trans. Amer. Math. Soc." }

 %ACM
 @String{CACM = "Communications of the {ACM}" }
 @String{CACM = "Commun. {ACM}" }
 @String{CompServ = "Comput. Surveys" }
 @String{JACM = "J. ACM" }
 @String{ACMMathSoft = "{ACM} Transactions on Mathematical Software" }
 @String{ACMMathSoft = "{ACM} Trans. Math. Software" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newsletter" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newslett." }

 @String{AmerSocio = "American Journal of Sociology" }
 @String{AmerStatAssoc = "Journal of the American Statistical Association" }
 @String{AmerStatAssoc = "J. Amer. Statist. Assoc." }
 @String{ApplMathComp = "Applied Mathematics and Computation" }
 @String{ApplMathComp = "Appl. Math. Comput." }
 @String{AmerMathMonthly = "American Mathematical Monthly" }
 @String{AmerMathMonthly = "Amer. Math. Monthly" }
 @String{BIT = "{BIT}" }
 @String{BritStatPsych = "British Journal of Mathematical and Statistical
          Psychology" }
 @String{BritStatPsych = "Brit. J. Math. Statist. Psych." }
 @String{CanMathBull = "Canadian Mathematical Bulletin" }
 @String{CanMathBull = "Canad. Math. Bull." }
 @String{CompApplMath = "Journal of Computational and Applied Mathematics" }
 @String{CompApplMath = "J. Comput. Appl. Math." }
 @String{CompPhys = "Journal of Computational Physics" }
 @String{CompPhys = "J. Comput. Phys." }
 @String{CompStruct = "Computers and Structures" }
 @String{CompStruct = "Comput. \& Structures" }
 @String{CompJour = "The Computer Journal" }
 @String{CompJour = "Comput. J." }
 @String{CompSysSci = "Journal of Computer and System Sciences" }
 @String{CompSysSci = "J. Comput. System Sci." }
 @String{Computing = "Computing" }
 @String{ContempMath = "Contemporary Mathematics" }
 @String{ContempMath = "Contemp. Math." }
 @String{Crelle = "Crelle's Journal" }
 @String{GiornaleMath = "Giornale di Mathematiche" }
 @String{GiornaleMath = "Giorn. Mat." } % didn't find in AMS MR., ibid.

 %IEEE
 @String{Computer = "{IEEE} Computer" }
 @String{IEEETransComp = "{IEEE} Transactions on Computers" }
 @String{IEEETransComp = "{IEEE} Trans. Comput." }
 @String{IEEETransAC = "{IEEE} Transactions on Automatic Control" }
 @String{IEEETransAC = "{IEEE} Trans. Automat. Control" }
 @String{IEEESpec = "{IEEE} Spectrum" } % didn't find in AMS MR
 @String{ProcIEEE = "Proceedings of the {IEEE}" }
 @String{ProcIEEE = "Proc. {IEEE}" } % didn't find in AMS MR
 @String{IEEETransAeroElec = "{IEEE} Transactions on Aerospace and Electronic
     Systems" }
 @String{IEEETransAeroElec = "{IEEE} Trans. Aerospace Electron. Systems" }

 @String{IMANumerAna = "{IMA} Journal of Numerical Analysis" }
 @String{IMANumerAna = "{IMA} J. Numer. Anal." }
 @String{InfProcLet = "Information Processing Letters" }
 @String{InfProcLet = "Inform. Process. Lett." }
 @String{InstMathApp = "Journal of the Institute of Mathematics and
     its Applications" }
 @String{InstMathApp = "J. Inst. Math. Appl." }
 @String{IntControl = "International Journal of Control" }
 @String{IntControl = "Internat. J. Control" }
 @String{IntNumerEng = "International Journal for Numerical Methods in
     Engineering" }
 @String{IntNumerEng = "Internat. J. Numer. Methods Engrg." }
 @String{IntSuper = "International Journal of Supercomputing Applications" }
 @String{IntSuper = "Internat. J. Supercomputing Applic." } % didn't find
%% in AMS MR
 @String{Kibernetika = "Kibernetika" }
 @String{JResNatBurStand = "Journal of Research of the National Bureau
     of Standards" }
 @String{JResNatBurStand = "J. Res. Nat. Bur. Standards" }
 @String{LinAlgApp = "Linear Algebra and its Applications" }
 @String{LinAlgApp = "Linear Algebra Appl." }
 @String{MathAnaAppl = "Journal of Mathematical Analysis and Applications" }
 @String{MathAnaAppl = "J. Math. Anal. Appl." }
 @String{MathAnnalen = "Mathematische Annalen" }
 @String{MathAnnalen = "Math. Ann." }
 @String{MathPhys = "Journal of Mathematical Physics" }
 @String{MathPhys = "J. Math. Phys." }
 @String{MathComp = "Mathematics of Computation" }
 @String{MathComp = "Math. Comp." }
 @String{MathScand = "Mathematica Scandinavica" }
 @String{MathScand = "Math. Scand." }
 @String{TablesAidsComp = "Mathematical Tables and Other Aids to Computation" }
 @String{TablesAidsComp = "Math. Tables Aids Comput." }
 @String{NumerMath = "Numerische Mathematik" }
 @String{NumerMath = "Numer. Math." }
 @String{PacificMath = "Pacific Journal of Mathematics" }
 @String{PacificMath = "Pacific J. Math." }
 @String{ParDistComp = "Journal of Parallel and Distributed Computing" }
 @String{ParDistComp = "J. Parallel and Distrib. Comput." } % didn't find
%% in AMS MR
 @String{ParComputing = "Parallel Computing" }
 @String{ParComputing = "Parallel Comput." }
 @String{PhilMag = "Philosophical Magazine" }
 @String{PhilMag = "Philos. Mag." }
 @String{ProcNAS = "Proceedings of the National Academy of Sciences
                    of the USA" }
 @String{ProcNAS = "Proc. Nat. Acad. Sci. U. S. A." }
 @String{Psychometrika = "Psychometrika" }
 @String{QuartMath = "Quarterly Journal of Mathematics, Oxford, Series (2)" }
 @String{QuartMath = "Quart. J. Math. Oxford Ser. (2)" }
 @String{QuartApplMath = "Quarterly of Applied Mathematics" }
 @String{QuartApplMath = "Quart. Appl. Math." }
 @String{RevueInstStat = "Review of the International Statisical Institute" }
 @String{RevueInstStat = "Rev. Inst. Internat. Statist." }

 %SIAM
 @String{JSIAM = "Journal of the Society for Industrial and Applied
     Mathematics" }
 @String{JSIAM = "J. Soc. Indust. Appl. Math." }
 @String{JSIAMB = "Journal of the Society for Industrial and Applied
     Mathematics, Series B, Numerical Analysis" }
 @String{JSIAMB = "J. Soc. Indust. Appl. Math. Ser. B Numer. Anal." }
 @String{SIAMAlgMeth = "{SIAM} Journal on Algebraic and Discrete Methods" }
 @String{SIAMAlgMeth = "{SIAM} J. Algebraic Discrete Methods" }
 @String{SIAMAppMath = "{SIAM} Journal on Applied Mathematics" }
 @String{SIAMAppMath = "{SIAM} J. Appl. Math." }
 @String{SIAMComp = "{SIAM} Journal on Computing" }
 @String{SIAMComp = "{SIAM} J. Comput." }
 @String{SIAMMatrix = "{SIAM} Journal on Matrix Analysis and Applications" }
 @String{SIAMMatrix = "{SIAM} J. Matrix Anal. Appl." }
 @String{SIAMNumAnal = "{SIAM} Journal on Numerical Analysis" }
 @String{SIAMNumAnal = "{SIAM} J. Numer. Anal." }
 @String{SIAMReview = "{SIAM} Review" }
 @String{SIAMReview = "{SIAM} Rev." }
 @String{SIAMSciStat = "{SIAM} Journal on Scientific and Statistical
     Computing" }
 @String{SIAMSciStat = "{SIAM} J. Sci. Statist. Comput." }

 @String{SoftPracExp = "Software Practice and Experience" }
 @String{SoftPracExp = "Software Prac. Experience" } % didn't find in AMS MR
 @String{StatScience = "Statistical Science" }
 @String{StatScience = "Statist. Sci." }
 @String{Techno = "Technometrics" }
 @String{USSRCompMathPhys = "{USSR} Computational Mathematics and Mathematical
     Physics" }
 @String{USSRCompMathPhys = "{U. S. S. R.} Comput. Math. and Math. Phys." }
 @String{VLSICompSys = "Journal of {VLSI} and Computer Systems" }
 @String{VLSICompSys = "J. {VLSI} Comput. Syst." }
 @String{ZAngewMathMech = "Zeitschrift fur Angewandte Mathematik und
     Mechanik" }
 @String{ZAngewMathMech = "Z. Angew. Math. Mech." }
 @String{ZAngewMathPhys = "Zeitschrift fur Angewandte Mathematik und Physik" }
 @String{ZAngewMathPhys = "Z. Angew. Math. Phys." }

% Publishers % ================================================= |

 @String{Academic = "Academic Press" }
 @String{ACMPress = "{ACM} Press" }
 @String{AdamHilger = "Adam Hilger" }
 @String{AddisonWesley = "Addison-Wesley" }
 @String{AllynBacon = "Allyn and Bacon" }
 @String{AMS = "American Mathematical Society" }
 @String{Birkhauser = "Birkha{\"u}ser" }
 @String{CambridgePress = "Cambridge University Press" }
 @String{Chelsea = "Chelsea" }
 @String{ClaredonPress = "Claredon Press" }
 @String{DoverPub = "Dover Publications" }
 @String{Eyolles = "Eyolles" }
 @String{HoltRinehartWinston = "Holt, Rinehart and Winston" }
 @String{Interscience = "Interscience" }
 @String{JohnsHopkinsPress = "The Johns Hopkins University Press" }
 @String{JohnWileySons = "John Wiley and Sons" }
 @String{Macmillan = "Macmillan" }
 @String{MathWorks = "The Math Works Inc." }
 @String{McGrawHill = "McGraw-Hill" }
 @String{NatBurStd = "National Bureau of Standards" }
 @String{NorthHolland = "North-Holland" }
 @String{OxfordPress = "Oxford University Press" }  %address Oxford or London?
 @String{PergamonPress = "Pergamon Press" }
 @String{PlenumPress = "Plenum Press" }
 @String{PrenticeHall = "Prentice-Hall" }
 @String{SIAMPub = "{SIAM} Publications" }
 @String{Springer = "Springer-Verlag" }
 @String{TexasPress = "University of Texas Press" }
 @String{VanNostrand = "Van Nostrand" }
 @String{WHFreeman = "W. H. Freeman and Co." }

%Entries
@article{ding2020more,
  title={Be more with less: Hypergraph attention networks for inductive text classification},
  author={Ding, Kaize and Wang, Jianling and Li, Jundong and Li, Dingcheng and Liu, Huan},
  journal={arXiv preprint arXiv:2011.00387},
  year={2020}
}
@inproceedings{lee2019set,
  title={Set transformer: A framework for attention-based permutation-invariant neural networks},
  author={Lee, Juho and Lee, Yoonho and Kim, Jungtaek and Kosiorek, Adam and Choi, Seungjin and Teh, Yee Whye},
  booktitle={International Conference on Machine Learning},
  pages={3744--3753},
  year={2019},
  organization={PMLR}
}
@inproceedings{rakesh2018linked,
  title={Linked causal variational autoencoder for inferring paired spillover effects},
  author={Rakesh, Vineeth and Guo, Ruocheng and Moraffah, Raha and Agarwal, Nitin and Liu, Huan},
  booktitle={Proceedings of the 27th ACM International Conference on Information and Knowledge Management},
  pages={1679--1682},
  year={2018}
}
@article{pritchard2000inference,
  title={Inference of population structure using multilocus genotype data},
  author={Pritchard, Jonathan K and Stephens, Matthew and Donnelly, Peter},
  journal={Genetics},
  volume={155},
  number={2},
  pages={945--959},
  year={2000},
  publisher={Oxford University Press}
}
@article{BART,
  title={Bayesian nonparametric modeling for causal inference},
  author={Hill, Jennifer L},
  journal={Journal of Computational and Graphical Statistics},
  volume={20},
  number={1},
  year={2011}
}
@article{willmott2005advantages,
  title={Advantages of the mean absolute error (MAE) over the root mean square error (RMSE) in assessing average model performance},
  author={Willmott, Cort J and Matsuura, Kenji},
  journal={Climate research},
  volume={30},
  number={1},
  pages={79--82},
  year={2005}
}
@inproceedings{guo2020learning,
  title={Learning individual causal effects from networked observational data},
  author={Guo, Ruocheng and Li, Jundong and Liu, Huan},
  booktitle={Proceedings of the 13th International Conference on Web Search and Data Mining},
  pages={232--240},
  year={2020}
}
@inproceedings{ma2021causal,
  title={Causal Inference under Networked Interference and Intervention Policy Enhancement},
  author={Ma, Yunpu and Tresp, Volker},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={3700--3708},
  year={2021},
  organization={PMLR}
}
@article{rubin1980randomization,
  title={Randomization analysis of experimental data: The Fisher randomization test comment},
  author={Rubin, Donald B},
  journal={Journal of the American Statistical Association},
  volume={75},
  number={371},
  pages={591--593},
  year={1980},
  publisher={JSTOR}
}
@inproceedings{CEVAE,
  title={Causal effect inference with deep latent-variable models},
  author={Louizos, Christos and Shalit, Uri and Mooij, Joris M and Sontag, David and Zemel, Richard and Welling, Max},
  booktitle={Advances in Neural Information Processing Systems},
  year={2017}
}
@inproceedings{CFR,
  title={Estimating individual treatment effect: generalization bounds and algorithms},
  author={Shalit, Uri and Johansson, Fredrik D and Sontag, David},
  booktitle={International Conference on Machine Learning},
  year={2017}
}
@inproceedings{netDeconf,
  title={Learning individual causal effects from networked observational data},
  author={Guo, Ruocheng and Li, Jundong and Liu, Huan},
  booktitle={ACM International Conference on Web Search and Data Mining},
  year={2020}
}
@article{kipf2016semi,
  title={Semi-supervised classification with graph convolutional networks},
  author={Kipf, Thomas N and Welling, Max},
  journal={arXiv preprint arXiv:1609.02907},
  year={2016}
}
@inproceedings{morris2019weisfeiler,
  title={Weisfeiler and leman go neural: Higher-order graph neural networks},
  author={Morris, Christopher and Ritzert, Martin and Fey, Matthias and Hamilton, William L and Lenssen, Jan Eric and Rattan, Gaurav and Grohe, Martin},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  number={01},
  pages={4602--4609},
  year={2019}
}
@inproceedings{gretton2005measuring,
  title={Measuring statistical dependence with Hilbert-Schmidt norms},
  author={Gretton, Arthur and Bousquet, Olivier and Smola, Alex and Sch{\"o}lkopf, Bernhard},
  booktitle={International conference on algorithmic learning theory},
  pages={63--77},
  year={2005},
  organization={Springer}
}
@article{bai2021hypergraph,
  title={Hypergraph convolution and hypergraph attention},
  author={Bai, Song and Zhang, Feihu and Torr, Philip HS},
  journal={Pattern Recognition},
  volume={110},
  pages={107637},
  year={2021},
  publisher={Elsevier}
}
@inproceedings{maas2013rectifier,
  title={Rectifier nonlinearities improve neural network acoustic models},
  author={Maas, Andrew L and Hannun, Awni Y and Ng, Andrew Y and others},
  booktitle={Proc. icml},
  volume={30},
  number={1},
  pages={3},
  year={2013},
  organization={Citeseer}
}
@inproceedings{sun2015causal,
  title={Causal inference via sparse additive models with application to online advertising},
  author={Sun, Wei and Wang, Pengyuan and Yin, Dawei and Yang, Jian and Chang, Yi},
  booktitle={AAAI Conference on Artificial Intelligence},
  year={2015}
}
@article{chernozhukov2021causal,
  title={Causal impact of masks, policies, behavior on early covid-19 pandemic in the US},
  author={Chernozhukov, Victor and Kasahara, Hiroyuki and Schrimpf, Paul},
  journal={Journal of econometrics},
  volume={220},
  number={1},
  pages={23--62},
  year={2021},
  publisher={Elsevier}
}
@article{varian2016causal,
  title={Causal inference in economics and marketing},
  author={Varian, Hal R},
  journal={Proceedings of the National Academy of Sciences},
  volume={113},
  number={27},
  pages={7310--7315},
  year={2016},
  publisher={National Acad Sciences}
}
@article{fisher1936design,
  title={Design of experiments},
  author={Fisher, Ronald Aylmer},
  journal={Br Med J},
  volume={1},
  number={3923},
  pages={554--554},
  year={1936},
  publisher={British Medical Journal Publishing Group}
}
@article{splawa1990application,
  title={On the application of probability theory to agricultural experiments. Essay on principles. Section 9.},
  author={Splawa-Neyman, Jerzy and Dabrowska, Dorota M and Speed, TP},
  journal={Statistical Science},
  pages={465--472},
  year={1990},
  publisher={JSTOR}
}
@article{aronow2017estimating,
  title={Estimating average causal effects under general interference, with application to a social network experiment},
  author={Aronow, Peter M and Samii, Cyrus},
  journal={The Annals of Applied Statistics},
  volume={11},
  number={4},
  pages={1912--1947},
  year={2017},
  publisher={Institute of Mathematical Statistics}
}
@article{basse2018analyzing,
  title={Analyzing two-stage experiments in the presence of interference},
  author={Basse, Guillaume and Feller, Avi},
  journal={Journal of the American Statistical Association},
  volume={113},
  number={521},
  pages={41--55},
  year={2018},
  publisher={Taylor \& Francis}
}
@article{imai2020causal,
  title={Causal inference with interference and noncompliance in two-stage randomized experiments},
  author={Imai, Kosuke and Jiang, Zhichao and Malani, Anup},
  journal={Journal of the American Statistical Association},
  pages={1--13},
  year={2020},
  publisher={Taylor \& Francis}
}
@inproceedings{kohavi2013online,
  title={Online controlled experiments at large scale},
  author={Kohavi, Ron and Deng, Alex and Frasca, Brian and Walker, Toby and Xu, Ya and Pohlmann, Nils},
  booktitle={Proceedings of the 19th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={1168--1176},
  year={2013}
}
@article{tchetgen2012causal,
  title={On causal inference in the presence of interference},
  author={Tchetgen, Eric J Tchetgen and VanderWeele, Tyler J},
  journal={Statistical methods in medical research},
  volume={21},
  number={1},
  pages={55--75},
  year={2012},
  publisher={Sage Publications Sage UK: London, England}
}
@inproceedings{ugander2013graph,
  title={Graph cluster randomization: Network exposure to multiple universes},
  author={Ugander, Johan and Karrer, Brian and Backstrom, Lars and Kleinberg, Jon},
  booktitle={Proceedings of the 19th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={329--337},
  year={2013}
}
@inproceedings{yuan2021causal,
  title={Causal Network Motifs: Identifying Heterogeneous Spillover Effects in A/B Tests},
  author={Yuan, Yuan and Altenburger, Kristen and Kooti, Farshad},
  booktitle={Proceedings of the Web Conference 2021},
  pages={3359--3370},
  year={2021}
}
@article{ahluwalia2001moderating,
  title={The moderating role of commitment on the spillover effect of marketing communications},
  author={Ahluwalia, Rohini and Unnava, H Rao and Burnkrant, Robert E},
  journal={Journal of Marketing research},
  volume={38},
  number={4},
  pages={458--470},
  year={2001},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}
@article{yilmaz2002geographic,
  title={Geographic and network neighbors: Spillover effects of telecommunications infrastructure},
  author={Yilmaz, Serdar and Haynes, Kingley E and Dinc, Mustafa},
  journal={Journal of Regional Science},
  volume={42},
  number={2},
  pages={339--360},
  year={2002},
  publisher={Wiley Online Library}
}
@article{zeng2019exploration,
  title={Exploration on the spatial spillover effect of infrastructure network on urbanization: A case study in Wuhan urban agglomeration},
  author={Zeng, Chen and Song, Yan and Cai, Dawei and Hu, Peiying and Cui, Huatai and Yang, Jing and Zhang, Hongxia},
  journal={Sustainable Cities and Society},
  volume={47},
  pages={101476},
  year={2019},
  publisher={Elsevier}
}
@article{benson2018simplicial,
  title={Simplicial closure and higher-order link prediction},
  author={Benson, Austin R and Abebe, Rediet and Schaub, Michael T and Jadbabaie, Ali and Kleinberg, Jon},
  journal={Proceedings of the National Academy of Sciences},
  volume={115},
  number={48},
  pages={E11221--E11230},
  year={2018},
  publisher={National Acad Sciences}
}
@inproceedings{feng2019hypergraph,
  title={Hypergraph neural networks},
  author={Feng, Yifan and You, Haoxuan and Zhang, Zizhao and Ji, Rongrong and Gao, Yue},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  number={01},
  pages={3558--3565},
  year={2019}
}
@article{yadati2018hypergcn,
  title={Hypergcn: Hypergraph convolutional networks for semi-supervised classification},
  author={Yadati, Naganand and Nimishakavi, Madhav and Yadav, Prateek and Louis, Anand and Talukdar, Partha},
  journal={arXiv preprint arXiv:1809.02589},
  volume={22},
  year={2018}
}
@article{zhang2019hyper,
  title={Hyper-SAGNN: a self-attention based graph neural network for hypergraphs},
  author={Zhang, Ruochi and Zou, Yuesong and Ma, Jian},
  journal={arXiv preprint arXiv:1911.02613},
  year={2019}
}
@inproceedings{jiang2019dynamic,
  title={Dynamic Hypergraph Neural Networks.},
  author={Jiang, Jianwen and Wei, Yuxuan and Feng, Yifan and Cao, Jingxuan and Gao, Yue},
  booktitle={IJCAI},
  pages={2635--2641},
  year={2019}
}
@book{brandes2013social,
  title={Social networks},
  author={Brandes, Ulrik and Freeman, Linton C and Wagner, Dorothea},
  year={2013}
}
@article{coclite2005traffic,
  title={Traffic flow on a road network},
  author={Coclite, Giuseppe Maria and Garavello, Mauro and Piccoli, Benedetto},
  journal={SIAM journal on mathematical analysis},
  volume={36},
  number={6},
  pages={1862--1886},
  year={2005},
  publisher={SIAM}
}
@article{alm2003biological,
  title={Biological networks},
  author={Alm, Eric and Arkin, Adam P},
  journal={Current opinion in structural biology},
  volume={13},
  number={2},
  pages={193--202},
  year={2003},
  publisher={Elsevier}
}
@article{velivckovic2017graph,
  title={Graph attention networks},
  author={Veli{\v{c}}kovi{\'c}, Petar and Cucurull, Guillem and Casanova, Arantxa and Romero, Adriana and Lio, Pietro and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1710.10903},
  year={2017}
}
@inproceedings{fatemi2020minimizing,
  title={Minimizing interference and selection bias in network experiment design},
  author={Fatemi, Zahra and Zheleva, Elena},
  booktitle={International AAAI Conference on Web and Social Media},
  year={2020}
}
@inproceedings{bhattacharya2020causal,
  title={Causal inference under interference and network uncertainty},
  author={Bhattacharya, Rohit and Malinsky, Daniel and Shpitser, Ilya},
  booktitle={Uncertainty in Artificial Intelligence},
  year={2020}
}
@inproceedings{li2013link,
  title={Link prediction in social networks based on hypergraph},
  author={Li, Dong and Xu, Zhiming and Li, Sheng and Sun, Xin},
  booktitle={Proceedings of the 22nd International Conference on World Wide Web},
  pages={41--42},
  year={2013}
}
@inproceedings{xu2013hyperlink,
  title={Hyperlink prediction in hypernetworks using latent social features},
  author={Xu, Ye and Rockmore, Dan and Kleinbaum, Adam M},
  booktitle={International Conference on Discovery Science},
  pages={324--339},
  year={2013},
  organization={Springer}
}
@article{yadati2018link,
  title={Link prediction in hypergraphs using graph convolutional networks},
  author={Yadati, Naganand and Nitin, Vikram and Nimishakavi, Madhav and Yadav, Prateek and Louis, Anand and Talukdar, Partha},
  year={2018}
}
@inproceedings{zhang2018beyond,
  title={Beyond link prediction: Predicting hyperlinks in adjacency space},
  author={Zhang, Muhan and Cui, Zhicheng and Jiang, Shali and Chen, Yixin},
  booktitle={Thirty-Second AAAI Conference on Artificial Intelligence},
  year={2018}
}
@inproceedings{arya2018exploiting,
  title={Exploiting relational information in social networks using geometric deep learning on hypergraphs},
  author={Arya, Devanshu and Worring, Marcel},
  booktitle={Proceedings of the 2018 ACM on International Conference on Multimedia Retrieval},
  pages={117--125},
  year={2018}
}
@inproceedings{benson2018sequences,
  title={Sequences of sets},
  author={Benson, Austin R and Kumar, Ravi and Tomkins, Andrew},
  booktitle={Proceedings of the 24th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={1148--1157},
  year={2018}
}
@inproceedings{huang2015scalable,
  title={Scalable hypergraph learning and processing},
  author={Huang, Jin and Zhang, Rui and Yu, Jeffrey Xu},
  booktitle={2015 IEEE International Conference on Data Mining},
  pages={775--780},
  year={2015},
  organization={IEEE}
}
@article{sharma2014predicting,
  title={Predicting multi-actor collaborations using hypergraphs},
  author={Sharma, Ankit and Srivastava, Jaideep and Chandra, Abhishek},
  journal={arXiv preprint arXiv:1401.6404},
  year={2014}
}
@article{goldstein2018ethical,
  title={Ethical issues in pragmatic randomized controlled trials: a review of the recent literature identifies gaps in ethical argumentation},
  author={Goldstein, Cory E and Weijer, Charles and Brehaut, Jamie C and Fergusson, Dean A and Grimshaw, Jeremy M and Horn, Austin R and Taljaard, Monica},
  journal={BMC Medical Ethics},
  year={2018},
  publisher={BioMed Central}
}
@article{luong2015effective,
  title={Effective approaches to attention-based neural machine translation},
  author={Luong, Minh-Thang and Pham, Hieu and Manning, Christopher D},
  journal={arXiv preprint arXiv:1508.04025},
  year={2015}
}
@inproceedings{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, Lukasz and Polosukhin, Illia},
  booktitle={Advances in Neural Information Processing Systems},
  year={2017}
}
@inproceedings{yoon2020much,
  title={How Much and When Do We Need Higher-order Information in Hypergraphs? A Case Study on Hyperedge Prediction},
  author={Yoon, Se-eun and Song, Hyungseok and Shin, Kijung and Yi, Yung},
  booktitle={Proceedings of The Web Conference 2020},
  pages={2627--2633},
  year={2020}
}
@article{mastrandrea2015contact,
  title={Contact patterns in a high school: a comparison between data collected using wearable sensors, contact diaries and friendship surveys},
  author={Mastrandrea, Rossana and Fournet, Julie and Barrat, Alain},
  journal={PloS one},
  volume={10},
  number={9},
  pages={e0136497},
  year={2015},
  publisher={Public Library of Science San Francisco, CA USA}
}
@article{chodrow2021hypergraph,
  title={Hypergraph clustering: from blockmodels to modularity},
  author={Chodrow, Philip S and Veldt, Nate and Benson, Austin R},
  journal={arXiv e-prints},
  pages={arXiv--2101},
  year={2021}
}
@inproceedings{wan2018item,
  title={Item recommendation on monotonic behavior chains},
  author={Wan, Mengting and McAuley, Julian},
  booktitle={Proceedings of the 12th ACM conference on recommender systems},
  pages={86--94},
  year={2018}
}
@inproceedings{wan2019fine,
  title={Fine-Grained Spoiler Detection from Large-Scale Review Corpora},
  author={Wan, Mengting and Misra, Rishabh and Nakashole, Ndapandula and McAuley, Julian},
  booktitle={Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
  pages={2605--2610},
  year={2019}
}
@article{hudgens2008toward,
  title={Toward causal inference with interference},
  author={Hudgens, Michael G and Halloran, M Elizabeth},
  journal={Journal of the American Statistical Association},
  volume={103},
  number={482},
  pages={832--842},
  year={2008},
  publisher={Taylor \& Francis}
}
@article{yao2018representation,
  title={Representation learning for treatment effect estimation from observational data},
  author={Yao, Liuyi and Li, Sheng and Li, Yaliang and Huai, Mengdi and Gao, Jing and Zhang, Aidong},
  journal={Advances in Neural Information Processing Systems},
  volume={31},
  year={2018}
}
@inproceedings{arbour2016inferring,
  title={Inferring network effects from observational data},
  author={Arbour, David and Garant, Dan and Jensen, David},
  booktitle={Proceedings of the 22nd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
  pages={715--724},
  year={2016}
}
@article{tchetgen2021auto,
  title={Auto-g-computation of causal effects on a network},
  author={Tchetgen Tchetgen, Eric J and Fulcher, Isabel R and Shpitser, Ilya},
  journal={Journal of the American Statistical Association},
  volume={116},
  number={534},
  pages={833--844},
  year={2021},
  publisher={Taylor \& Francis}
}
@article{zigler2021bipartite,
  title={Bipartite causal inference with interference},
  author={Zigler, Corwin M and Papadogeorgou, Georgia},
  journal={Statistical science: a review journal of the Institute of Mathematical Statistics},
  volume={36},
  number={1},
  pages={109},
  year={2021},
  publisher={NIH Public Access}
}
@article{pouget2019variance,
  title={Variance reduction in bipartite experiments through correlation clustering},
  author={Pouget-Abadie, Jean and Aydin, Kevin and Schudy, Warren and Brodersen, Kay and Mirrokni, Vahab},
  year={2019}
}
@inproceedings{karrer2021network,
  title={Network experimentation at scale},
  author={Karrer, Brian and Shi, Liang and Bhole, Monica and Goldman, Matt and Palmer, Tyrone and Gelman, Charlie and Konutgan, Mikael and Sun, Feng},
  booktitle={Proceedings of the 27th ACM SIGKDD Conference on Knowledge Discovery \& Data Mining},
  pages={3106--3116},
  year={2021}
}

==> theory.tex <==
\subsection{Theory}
In this subsection, we give theoretic analysis for the identifiability of the individual treatment effect under the existence of spillover effect in hypergraphs. First, we list some definitions and necessary assumptions in this work.

% the list may be repeated
First, we denote the set of all the hyperedges which have interference to node $i$ (e.g., the hyperedges which contains node $i$, i.e., $\mathcal{E}_i$) as $\mathcal{E}^s_i$, and denote the set of nodes contained in at least one of the hyperedges in $\mathcal{E}^s_i$ as $\mathcal{V}^s_i$ (e.g., the set of node $i$'s neighboring nodes). We use  $\mathcal{V}^s_i-\{i\}$ to denote the set of nodes in $\mathcal{V}^s_i$ except $i$ itself. 
We denote a summary function $\mathtt{SMR}(\cdot)$ which takes $\mathcal{E}^s_i$, the treatment assignment of nodes in $\mathcal{V}^s_i-\{i\}$ (denoted by $\mathbf{T}_{\mathcal{V}^s_i-\{i\}}$), and the instance features of these nodes (denoted by $\mathbf{X}_{\mathcal{V}^s_i-\{i\}}$) as input, and maps them into a vector $\mathbf{o}_i$: 
%For simplicity, we denote the list of nodes which influence node $i$ as $\mathcal{N}_i$ (not including node $i$ itself), and 
%We denote the summary function $\mathtt{SMR}(\cdot): \mathcal{X}^{|\mathcal{N}_i| \times d} \times \{0,1\}^{|\mathcal{N}_i|} \rightarrow \mathcal{S}$ over their covariates and treatment assignments is denoted by:
% \begin{equation}
%     \mathbf{s}_i = \mathtt{SMR}(\mathbf{X}_{\mathcal{N}_i}, \mathbf{T}_{\mathcal{N}_i})
% \end{equation}
\begin{equation}
     \mathbf{o}_i = \mathtt{SMR}(\mathcal{E}^s_i, \mathbf{X}_{\mathcal{V}^s_i-\{i\}}, \mathbf{T}_{\mathcal{V}^s_i-\{i\}})
 \end{equation}
%Then the potential outcome under treatment $t_i$, $\mathbf{x}_i$ and summary $\mathbf{s}_i$ is denoted by $Y_i(t_i,\mathbf{x}_i,\mathbf{s}_i)$. 

\begin{assumption}
(Summary function) 
For any node $i\in[n]$, any values of $\mathcal{E}^s_i, {X}_{\mathcal{V}^s_i-\{i\}}$, and ${T}_{\mathcal{V}^s_i-\{i\}}$, if the output of summary function $\mathbf{o}_i$ is determined, then the value of the potential outcomes $y_i^{1}$ and $y_i^{0}$ with feature $\mathbf{x}_i$ are also determined. 
%For all the node $\forall i=1,...,n, \forall \mathbf{T}, \mathbf{T}' \in \{0,1\}^{n}, \forall \mathbf{X}, \mathbf{X}' \in \mathcal{X}^{n}$, if the summary function  $\mathtt{SMR}(\mathbf{X}_{\mathcal{N}_i},\mathbf{T}_{\mathcal{N}_i}, \mathcal{E}_i)=\mathtt{SMR}(\mathbf{X}'_{\mathcal{N}_i},\mathbf{T}'_{\mathcal{N}_i},\mathcal{E}_i)$, then the potential outcome $Y_i(t_i, \mathbf{T}, \mathbf{X})=Y_i(t_i, \mathbf{T}', \mathbf{X}')$.
\label{assumption:summary}
\end{assumption}

\begin{assumption}
(Unconfoundedness) For any node $i\in[n]$, given the features, the potential outcomes are independent with the treatment assignment and summary of neighbors, i.e., $Y_i^1,Y_i^0 \bigCI T_i, O_i | {X}_i$. \label{assumption:unconfoundeness}
\end{assumption}

Based on the above assumptions, the identification of potential outcomes $Y_i^{1}$ and $Y_i^{0}$ for each node $i$ can be proved (here we take $Y_i^{1}$ as an example):
% \begin{align}
% \mathbb{E}[Y_i|T_i = t_i, \mathbf{S}_i = \mathbf{s}_i, \mathbf{X}_i] &\overset{Asm. 1}{=} \mathbb{E}[Y_i(t_i,  \mathbf{s}_i)|T_i = t_i, \mathbf{S}_i = \mathbf{s}_i, \mathbf{X}_i]\\
% &\overset{Asm. 2}{=} \mathbb{E}[Y_i(t_i, \mathbf{s}_i))|\mathbf{X}_i]
% \end{align}
\begin{align}
Y_i^{1} \overset{(0)}{=}&\mathbb{E}[\Phi_Y(T_i=1, X_i=\mathbf{x}_i, T_{-i}=\mathbf{T}_{-i},{X}_{-i}=\mathbf{X}_{-i},H=\mathbf{H})] \\\overset{(1)}{=}& \mathbb{E}[\Phi_Y(T_i=1, X_i=\mathbf{x}_i, O_i=\mathbf{o}_i)) \\
\overset{(2)}{=} &\mathbb{E}[\Phi_Y(T_i=1, X_i=\mathbf{x}_i, O_i=\mathbf{o}_i)|X_i=\mathbf{x}_i] \\
\overset{(3)}{=} &\mathbb{E}[\Phi_Y(T_i=1, X_i=\mathbf{x}_i, O_i=\mathbf{o}_i)|X_i=\mathbf{x}_i, T_i=1,O_i=\mathbf{o}_i] \\
\overset{(4)}{=} &\mathbb{E}[Y_i|X_i, T_i=1,O_i=\mathbf{o}_i].
\end{align}
Here, the equation $(0)$ is based on the definition of potential outcome in this setting; equation $(1)$ is inferred from Assumption (1); equation (2) is a straightforward derivation; equation (3) is based on Assumption (2); and equation (4) is based on the widely used consistency assumption \cite{rubin1980randomization}. Based on the above proof for the identification of potential outcomes, the identification of ITE can be straightforwardly derived.

